Chinese Short-Form Creative Content Generation via Explanation-Oriented Multi-Objective Optimization

Chinese demonstrates high semantic compactness and rich metaphorical expressiveness, enabling limited text to convey dense meanings while increasing the difficulty of generation and verification, particularly in short-form creative natural language generation (CNLG). In the real world, users often require personalized, fine-grained creative constraints, making reliable verification critical to guiding optimization. According to Brunswik's Lens Model from psychology, constraints' achievement can be inferred from sufficient observable cues. Existing studies are mainly outcome-oriented, implicitly assuming that the outcome itself provides adequate cues for verification. However, this assumption breaks down in Chinese short-form CNLG (e.g., naming or advertising) with diverse personalized constraints, where extremely brief outcomes inherently offer limited information. Explanations can naturally serve as extra cues. Nevertheless, under complex constraints, LLMs' explanations may suffer from hallucination, incompleteness, or ambiguity. To address these, we novelly formalize the Chinese short-form CNLG task as a heterogeneous multi-objective optimization (HMO) issue that needs to jointly optimize multiple personalized constraints and explanation reliability. We further propose MAGIC-HMO, a training-free multi-agent framework that optimizes these objectives through iterative generation and verification under an explanation-oriented multi-objective strategy. Experiments on \emph{Chinese Baby Naming}, a challenging benchmark, demonstrate that MAGIC-HMO significantly outperforms six strong baselines across various LLM backbones. Relevant data and codes are available at https://github.com/foolfun/MAGIC_HMO.

==> algorithm/a3.tex <==
\begin{algorithm}[!t]
\caption{DI-HMOO}
\label{alg:di-hmoo}
\SetAlgoNlRelativeSize{0} % 行号字体大小
\scriptsize
\DontPrintSemicolon
  \KwIn{User input $x$, hybrid information $\mathcal{I}$}
  \KwOut{Creative output $\mathcal{Y}$ }
  \textbf{Dynamic Iterative Multi-Objective Optimization Stage} \\
   Initialize examples $I_{\text{shots}}$,
   generation round $j \gets 0$, 
   implicit evaluation round $j_{\text{imp}} \gets 0$,    
   explicit evaluation round $j_{\text{exp}} \gets 0$,
   max evaluation round $t_{\text{max}}$,
   warmup round $t_{\text{w}}$, 
   initial threshold $\delta$, 
   decay factor $\alpha$, 
   implicit rationality objective $\mathcal{O}_{\text{imp}} =\{o_\text{acc},o_\text{com},o_\text{cla}\}$,
   implicit multi-objective weights $W_{\text{imp}} \gets [0.5,0.5]$,
    explicit multi-objective weights $W_{\text{exp}}$,
   implicit history $\mathcal{H}_{\text{imp}} \gets \emptyset$,
    explicit history $\mathcal{H}_{\text{exp}} \gets \emptyset$,
    and the $j$-th step regenerate flag $l^{j} \gets \text{NULL}$ ($0$ is no regeneration and $1$ is regeneration).\;
   % 结束条件 通过评估或达到最大轮次
   \Repeat{\textnormal{$l^{j}$  is 0 or $j > t_{\text{max}}$.}}{
        % 生成结果
        \textbf{$A_\text{G}$ generate result}
            $\mathcal{Y}^{j} \gets A_\text{G}(x, I_{\text{rk}}, I_{\text{desc}}, I_{\text{reqs}}, I_{\text{shots}}, l^{j}, \mathcal{B}^{j})$ \\
         % 评估结果
        \textbf{$A_\text{E}$ evaluates result $\mathcal{Y}^{j}$}: \;
         \Indp
            % 设定当前阈值
            Setting thresholds and scores:
            $\psi^{j}_{\text{imp}}$, $\psi^{j}_{\text{exp}}$.\;
            Reset the $j$-th sores and feedback: $\theta^{j}_{\text{imp}} \gets \text{NULL}$, $\theta^{j}_{\text{exp}} \gets \text{NULL}$, $\mathcal{B}^{j} \gets \emptyset$. \;
             % 1隐式评估
            \textbf{a. Implicit evaluation}:  \;
            \Indp
                % 基于规则的准确性性评估
                $(l^{j},b_{j}) \gets F_{\text{acc}}(\mathcal{Y}^{j})$;  $\mathcal{B}^{j} \gets \mathcal{B}^{j} \cup \{b_{j}\}$.\;
                \textbf{if} \textnormal{$l^{j}$ is 1} \textbf{then}  $\mathcal{H}_{\text{imp}} \cup {\{(\mathcal{Y}^{j},\theta^{j}_{\text{imp}})\}}$; 
                    $j \gets j+1$; 
                    \textbf{continue}. \;
                % 完整性和清晰度的细粒度评估
                \ForEach{
                    \textnormal{$e^{j}_{k}$ in $\{e^{j}_{1},e^{j}_{2},\ldots,e^{j}_{m}\}$}
                }{ 
                    $(s^{j}_{\text{com}},s^{j}_{\text{cla}},b_{j}) \gets A_\text{E}(e^{j}_{k},u_{k},I_\text{type})$; \;
                    $\mathcal{S}^{j}_{\text{com}} \gets \mathcal{S}^{j}_{\text{com}} \cup \{s^{j}_{\text{com}}\}$; \;
                    $\mathcal{S}^{j}_{\text{cla}} \gets \mathcal{S}^{j}_{\text{cla}} \cup \{s^{j}_{\text{cla}}\}$; \;
                    $\mathcal{B}^{j} \gets \mathcal{B}^{j} \cup \{b_{j}\}$. \\                 
                }
                % 计算隐式最终得分
                $\mathcal{S}^{j}_{\text{imp}} = \{Norm(AVG(\mathcal{S}^{j}_{\text{com}})), Norm(AVG(\mathcal{S}^{j}_{\text{cla}}))\}$; \;
                $\theta^{j}_{\text{imp}} \gets W_{\text{imp}} \cdot \mathcal{S}^{j}_{\text{imp}}$.\;
                % 若低于阈值则重新生成
                 \textbf{if} $\theta^{j}_{\text{imp}} < \psi^{j}_{\text{imp}}$ 
                 \textbf{then} $l^{j} \gets 1$;
                    $\mathcal{H}_{\text{imp}}  \cup {\{(\mathcal{Y}^{j},\theta^{j}_{\text{imp}})\}}$; 
                     $j \gets j+1$; 
                    \textbf{continue}. \;
            \Indm
            % 2显式评估：
            \textbf{b. Explicit evaluation}: \;
                \Indp
                    % 任务相关性的细粒度评估
                     \ForEach{
                        \textnormal{$e^{j}_{k}$ in $\{e^{j}_{1},e^{j}_{2},\ldots,e^{j}_{m}\}$}
                     }{ 
                        $(s^{j}_{\text{exp}},b_{j}) \gets A_\text{E}(e^{j}_{k},q_{k},I_\text{rk})$; \;
                        $\mathcal{S}^{j}_{\text{exp}} \gets \mathcal{S}^{j}_{\text{exp}} \cup \{s^{j}_{\text{exp}}\}$; \;
                        $\mathcal{B}^{j} \gets \mathcal{B}^{j} \cup \{b_{j}\}$.                  
                    }
                    % 计算显式最终得分
                    $\theta^{j}_{\text{exp}} \gets W_{\text{exp}} \cdot Norm(S^{j}_{\text{exp}})$.\;
                    % 若低于阈值则重新生成
                    \If{}{
                           
                    }
                \textbf{if} $\theta^{j}_{\text{exp}} < \psi^{j}_{\text{exp}}$ 
                 \textbf{then} 
                  $l^{j} \gets 1$; 
                $\mathcal{H}_{\text{exp}}  \cup \{(\mathcal{Y}^{j},\theta^{j}_{\text{exp}})\}$; 
                $j \gets j+1$; 
                    \textbf{continue}. \;
                \Indm
                $l^{j} \gets 0$. \;
        \Indm
   }
   \textbf{if} \textnormal{$j < t_{\text{max}}$} \textbf{then} $\mathcal{Y} \gets \mathcal{Y}^{j}$. \;
   \textbf{else if} \textnormal{${H}_{\text{exp}}$ is not $\emptyset$} \textbf{then} Find best result $\mathcal{Y}$ from $\mathcal{H}_{\text{exp}}$. \;
    \textbf{else}  Find best result $\mathcal{Y}$ from $\mathcal{H}_{\text{imp}}$.
\end{algorithm}
